AIDBench: A benchmark for evaluating the authorship identification capability of large language models

As large language models (LLMs) rapidly advance and integrate into daily life, the privacy risks they pose are attracting increasing attention. We focus on a specific privacy risk where LLMs may help identify the authorship of anonymous texts, which challenges the effectiveness of anonymity in real-world systems such as anonymous peer review systems. To investigate these risks, we present AIDBench, a new benchmark that incorporates several author identification datasets, including emails, blogs, reviews, articles, and research papers. AIDBench utilizes two evaluation methods: one-to-one authorship identification, which determines whether two texts are from the same author; and one-to-many authorship identification, which, given a query text and a list of candidate texts, identifies the candidate most likely written by the same author as the query text. We also introduce a Retrieval-Augmented Generation (RAG)-based method to enhance the large-scale authorship identification capabilities of LLMs, particularly when input lengths exceed the models' context windows, thereby establishing a new baseline for authorship identification using LLMs. Our experiments with AIDBench demonstrate that LLMs can correctly guess authorship at rates well above random chance, revealing new privacy risks posed by these powerful models. The source code and data will be made publicly available after acceptance.

==> contents/Preliminaries.tex <==
\section{Related Work}
Our benchmark is related with the longstanding authorship attribution task \citep{stamatatos2009survey}, which is initially formulated as supervised authorship identification and recently addressed with LLMs.   
\subsection{Supervised Authorship Identification}
Early work uses text statistics such as n-grams, topic, or syntax as features~\citep{Koppel2007MeasuringDU, Sharma2018AnIO, Sundararajan2018WhatR, SeroussiTopicModel}, and then leverage SVM,  random forest or topic models to conduct authorship verification. Some work uses deep learning models like RNNs and CNNs to extract more complex features for authorship verification~\citep{Bagnall2015AuthorIU, benzebouchi2018multi, Ruder2016CharacterlevelAM}. Pretrained models such as BERT are also used to get text embeddings~\citep{HuertasTato2022PARTPA, Barlas2020CrossDomainAA, Fabien2020BertAAB, rivera-soto-etal-2021-learning} and one can verify the authorship of two texts by measuring the similarity of their embeddings.

\subsection{Authorship Identification by LLMs}
Due to the abilities of LLMs understanding texts and human instructions, researchers naturally explore using LLMs for authorship identification. \citep{Hung2023WhoWI} prompt LLMs with step-by-step stylometric explanations for  authorship verification. \citep{Huang2024CanLL} design various prompts with different levels of guidance and ask LLMs to conduct authorship verification and attribution in an end-to-end way. The guidance includes ignoring topics, ignoring content, and focusing on linguistic features. Nonetheless, they did not experiment with hard scenarios such as the same author with different topics, or different authors with the same topic. %In the authorship verification task, they give two anonymous texts and ask LLMs to distinguish whether they belong to the same author. For authorship attribution, they provide several known authors with a list of their writings and attempt to have the LLMs categorize a target text to one of the authors based on the provided information. 
%They provided certain guidance in the prompts, such as instructing it to ignore topics and content and focus on linguistic features, and demonstrated the effectiveness of these guidances.


Our paper extends previous work in several key aspects. We focus on an authorship identification task that mimics the anonymous paper review system by identifying the most likely texts from the same author. Additionally, our experiments cover a wider range of scenarios and demonstrate the behaviors of LLMs in various axes, including different context lengths and challenging scenarios.

==> contents/limitations_and_future_directions.tex <==
\section{Limitation and future directions}


The AIDBench offers a benchmark for assessing LLMs' authorship identification capabilities in scenarios closer to real-world anonymous review systems, highlighting significant privacy risks associated with anonymous systems. In this section, we address the potential limitations of AIDBench and outline future directions.

Firstly, it is worthy to note that due to cost constraints, we evaluated only a limited number of models. Additionally, large commercial models are continually emerging and evolving rapidly, such as the Gemini~\citep{team2023gemini}, Claude 3, Llama, Mistral families, and many others. Therefore, future exploration and evaluation of these models are warranted.

%(Gemini Ultra, Gemini Pro, Gemini Nano) (Claude 3 Opus, Claude 3 Sonnet, Claude 3 Haiku)

Another aspect to consider is that research papers often involve multiple authors, each contributing differently to the paper's writing. It would be intriguing to curate more nuanced subsets of research papers based on author positions, such as a first-author subset. This approach could provide insights into how author position affects the authorship identification problem in research papers. Additionally, in our experiments, we only utilize the abstract information of a paper. However, in the future, incorporating more detailed paper information could lead to a more accurate evaluation. %Another potential direction is to work directly with anonymous review datasets.

Furthermore, in the evaluation process, we employed only two types of prompts: the general prompt and the topic-ignored prompt. Recognizing the significant impact of prompt quality on model responses, it is essential for a more comprehensive exploration of LLMs' authorship identification capabilities that we develop a more nuanced set of prompts for future evaluation and analysis.

%Thirdly, during the evaluation process, we utilized only two types of prompts: the general prompt and the topic-ignored prompt. Given the close relationship between the quality of model responses and prompts, for a more in-depth exploration of LLMs' authorship identification capabilities, it is imperative that we design a more extensive and nuanced set of prompts for future evaluation and analysis.



Finally, the RAG-based approach we introduced enables LLMs with limited context windows to conduct authorship identification. To ensure the success of authorship identification, it's necessary to limit the candidate list obtained through RAG screening to a specific quantity. Additionally, we often encounter individual texts with considerable lengths. Therefore, a future direction of our work involves exploring methods to decompose long texts into shorter segments, indirectly facilitating comparisons between the original texts by comparing these shorter segments. One approach is to segment the long text into several shorter segments. In the one-to-two identification task, LLMs can compare pairs of these shorter segments, assigning scores during each comparison. Ultimately, scores are weighted and summed based on the length of each segment.

%Lastly, the RAG-based approach we proposed enables LLMs that do not support long-text inputs to perform authorship identification. However, to maintain the success rate of authorship identification, the candidate list obtained through RAG screening needs to be constrained to a certain quantity. Moreover, we often encounter individual texts with substantial lengths. Therefore, a future direction of our work is to attempt the decomposition of a long text into shorter texts, indirectly facilitating the comparison of the original texts through comparisons between the shorter texts. For instance, one direct idea involves segmenting the long text into several shorter segments. In the one-to-one identification task, LLMs can compare pairs of these shorter segments and assign scores during each comparison. Ultimately, scores are weighted and summed based on the length of each segment.


% Hiearchical comparison

% Thirdly, due to the insufficient attention from the community regarding the potent authorship identification capabilities of LLMs and their potential risks to various anonymization systems, we primarily relied on two common metrics, rank, and precision, in AIDbench. However, there is a necessity to enhance and expand the assessment criteria for evaluating LLMs' authorship identification capabilities. Further refinement and enrichment of these evaluation metrics are imperative.

==> table/ap_dataset.tex <==
\begin{table}[!h]
\centering 
\renewcommand{\arraystretch}{1.35}

% \normalsize
\label{tab:scenarios}
% \vspace{2pt}
\caption{Summary of the dataset used in AIDBench}
\resizebox{1.1\linewidth}{!}
{
\begin{tabular}{p{2.5cm}p{2.5cm}p{2cm}p{5.7cm}p{2.5cm}}
\toprule
\textbf{Dataset} & \textbf{Author Number} & \textbf{Text Number} & \textbf{Description} & \textbf{New or existing} \\
\midrule
Research Paper & $1,500$ & $15,000$ & We gathered computer science papers from arXiv\footnote{\url{https://arxiv.org}} to assess LLMs' authorship identification in real-world scenarios, potentially undermining the anonymity of peer review systems if successful. & \textbf{New} \\

Enron Email & $174$ & $500,000$ & The Enron email dataset is filtered to remove sender/receiver info and short emails, ensuring unbiased LLM assessment with a consistent set of authors and emails. & \citep{klimt2004enron} \\

Blog & $1,500$ & $15,000$ & The Blog Authorship Corpus contains posts from bloggers on blogger.com in August 2004, revealing author identities through linguistic patterns and writing styles. & \citep{Schler2006EffectsOA} \\

IMDb Review & $62$ & $3,100$ & The IMDb reviews data is sourced from the IMDb62 dataset. We analyzed 50 reviews for each of the 62 authors in our study. & \citep{Seroussi2011AuthorshipAW} \\

Guardian & $13$ & $650$ & The Guardian corpus dataset from The Guardian newspaper explores authorship attribution across genres and topics, with contributions from 13 authors. & \citep{guardian} \\

\bottomrule
\end{tabular}
}
\end{table}

==> table/ap_paper-eval-non-topic-ignored.tex <==
%%%% non topic ignore
\renewcommand{\arraystretch}{1.2}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{Evaluation result on Research Paper.Note: non-topic ignore}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c|cccc|cccc}
    \toprule
         & \multicolumn{4}{c}{\bf 2 authors} & \multicolumn{4}{c}{\bf 5 authors}  \\
         & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10} & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10}  \\
    \midrule
         GPT-3.5-turbo$^\diamondsuit$ & $\text{56.7}_{\pm \text{35.3}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{96.7}_{\pm \text{10.5}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{30.0}_{\pm \text{24.6}}$ & $\text{60.0}_{\pm \text{26.3}}$ & $\text{73.3}_{\pm \text{21.1}}$ & $\text{90.0}_{\pm \text{16.1}}$  \\
         GPT-4-turbo$^\diamondsuit$ & $\text{80.0}_{\pm \text{23.3}}$ & $\text{93.3}_{\pm \text{14.1}}$ & $\text{93.3}_{\pm \text{14.1}}$ & $\text{96.7}_{\pm \text{10.5}}$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{90.0}_{\pm \text{16.1}}$ & $\text{93.3}_{\pm \text{14.1}}$  \\ 
         Kimi$^\diamondsuit$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{93.3}_{\pm \text{14.1}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{50.0}_{\pm \text{17.6}}$ & $\text{63.3}_{\pm \text{10.5}}$ & $\text{73.3}_{\pm \text{14.1}}$ & $\text{76.7}_{\pm \text{16.1}}$  \\
         Baichuan-turbo-192k$^\diamondsuit$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{80.0}_{\pm \text{23.3}}$ & $\text{80.0}_{\pm \text{23.3}}$ & $\text{90.0}_{\pm \text{16.1}}$ & $\text{46.7}_{\pm \text{23.3}}$ & $\text{60.0}_{\pm \text{30.6}}$ & $\text{66.7}_{\pm \text{31.4}}$ & $\text{73.3}_{\pm \text{21.1}}$  \\
         Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{76.7}_{\pm \text{31.6}}$ & $\text{83.3}_{\pm \text{23.6}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{23.3}_{\pm \text{27.4}}$ & $\text{26.7}_{\pm \text{26.3}}$ & $\text{50.0}_{\pm \text{28.3}}$  \\
    \midrule
        & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} \\
    \midrule
         GPT-3.5-turbo$^\diamondsuit$ & $\text{56.7}_{\pm \text{35.3}}$ & $\text{55.6}_{\pm \text{18.9}}$ & $\text{55.3}_{\pm \text{12.6}}$ & $\text{52.3}_{\pm \text{6.7}}$ & $\text{30.0}_{\pm \text{24.6}}$ & $\text{25.6}_{\pm \text{16.6}}$ & $\text{20.0}_{\pm \text{10.4}}$ & $\text{18.7}_{\pm \text{7.1}}$  \\
         GPT-4-turbo$^\diamondsuit$ & $\text{80.0}_{\pm \text{23.3}}$ & $\text{72.2}_{\pm \text{15.9}}$ & $\text{70.0}_{\pm \text{15.8}}$ & $\text{59.7}_{\pm \text{11.5}}$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{64.4}_{\pm \text{20.8}}$ & $\text{53.3}_{\pm \text{18.6}}$ & $\text{39.7}_{\pm \text{13.8}}$  \\ 
         Kimi$^\diamondsuit$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{76.7}_{\pm \text{25.9}}$ & $\text{72.7}_{\pm \text{24.4}}$ & $\text{56.7}_{\pm \text{9.6}}$ & $\text{50.0}_{\pm \text{17.6}}$ & $\text{41.1}_{\pm \text{18.2}}$ & $\text{34.0}_{\pm \text{14.2}}$ & $\text{26.0}_{\pm \text{14.4}}$  \\
         Baichuan-turbo-192k$^\diamondsuit$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{68.9}_{\pm \text{22.1}}$ & $\text{64.7}_{\pm \text{20.4}}$ & $\text{58.7}_{\pm \text{16.3}}$ & $\text{46.7}_{\pm \text{23.3}}$ & $\text{43.3}_{\pm \text{27.4}}$ & $\text{43.3}_{\pm \text{25.0}}$ & $\text{39.3}_{\pm \text{20.8}}$  \\
         Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{70.0}_{\pm \text{29.2}}$ & $\text{50.0}_{\pm \text{23.6}}$ & $\text{45.3}_{\pm \text{14.0}}$ & $\text{47.0}_{\pm \text{8.1}}$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{10.0}_{\pm \text{14.3}}$ & $\text{7.3}_{\pm \text{9.1}}$ & $\text{8.3}_{\pm \text{5.7}}$  \\
    \midrule
        & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} \\
    \midrule
         GPT-3.5-turbo$^\diamondsuit$ & $\text{6.3}_{\pm \text{3.9}}$ & $\text{18.5}_{\pm \text{6.3}}$ & $\text{30.7}_{\pm \text{7.0}}$ & $\text{58.1}_{\pm \text{7.4}}$ & $\text{3.3}_{\pm \text{2.7}}$ & $\text{8.5}_{\pm \text{5.5}}$ & $\text{11.1}_{\pm \text{5.8}}$ & $\text{20.7}_{\pm \text{7.8}}$  \\
         GPT-4-turbo$^\diamondsuit$ & $\text{8.9}_{\pm \text{2.6}}$ & $\text{24.1}_{\pm \text{5.3}}$ & $\text{38.9}_{\pm \text{8.8}}$ & $\text{66.3}_{\pm \text{12.8}}$ & $\text{7.8}_{\pm \text{3.2}}$ & $\text{21.5}_{\pm \text{6.9}}$ & $\text{29.6}_{\pm \text{10.3}}$ & $\text{44.1}_{\pm \text{15.4}}$  \\ 
         Kimi$^\diamondsuit$ & $\text{9.6}_{\pm \text{1.9}}$ & $\text{25.6}_{\pm \text{8.6}}$ & $\text{40.4}_{\pm \text{13.6}}$ & $\text{62.9}_{\pm \text{10.6}}$ & $\text{5.6}_{\pm \text{2.0}}$ & $\text{13.7}_{\pm \text{6.1}}$ & $\text{18.9}_{\pm \text{7.9}}$ & $\text{28.9}_{\pm \text{16.0}}$  \\
         Baichuan-turbo-192k$^\diamondsuit$ & $\text{7.8}_{\pm \text{3.2}}$ & $\text{22.9}_{\pm \text{7.4}}$ & $\text{35.9}_{\pm \text{11.3}}$ & $\text{65.2}_{\pm \text{18.1}}$ & $\text{5.2}_{\pm \text{2.6}}$ & $\text{14.4}_{\pm \text{9.2}}$ & $\text{24.1}_{\pm \text{13.9}}$ & $\text{43.7}_{\pm \text{23.1}}$  \\
         Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{7.8}_{\pm \text{3.2}}$ & $\text{16.7}_{\pm \text{7.9}}$ & $\text{25.2}_{\pm \text{7.8}}$ & $\text{52.2}_{\pm \text{9.0}}$ & $\text{1.1}_{\pm \text{1.8}}$ & $\text{3.3}_{\pm \text{4.8}}$ & $\text{4.1}_{\pm \text{5.1}}$ & $\text{9.3}_{\pm \text{6.4}}$  \\
    \midrule
        & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} \\
    \midrule
         GPT-3.5-turbo$^\diamondsuit$ & $\text{11.3}_{\pm \text{7.1}}$ & $\text{27.8}_{\pm \text{9.4}}$ & $\text{39.5}_{\pm \text{9.0}}$ & $\text{55.1}_{\pm \text{7.0}}$ & $\text{6.0}_{\pm \text{4.9}}$ & $\text{12.8}_{\pm \text{8.3}}$ & $\text{14.3}_{\pm \text{7.4}}$ & $\text{19.6}_{\pm \text{7.4}}$  \\
         GPT-4-turbo$^\diamondsuit$ & $\text{16.0}_{\pm \text{4.7}}$ & $\text{36.1}_{\pm \text{8.0}}$ & $\text{50.0}_{\pm \text{11.3}}$ & $\text{62.8}_{\pm \text{12.1}}$ & $\text{14.0}_{\pm \text{5.8}}$ & $\text{32.2}_{\pm \text{10.4}}$ & $\text{38.1}_{\pm \text{13.3}}$ & $\text{41.8}_{\pm \text{14.6}}$  \\ 
         Kimi$^\diamondsuit$ & $\text{17.3}_{\pm \text{3.4}}$ & $\text{38.3}_{\pm \text{12.9}}$ & $\text{51.9}_{\pm \text{17.5}}$ & $\text{59.7}_{\pm \text{10.1}}$ & $\text{10.0}_{\pm \text{3.5}}$ & $\text{20.6}_{\pm \text{9.1}}$ & $\text{24.3}_{\pm \text{10.2}}$ & $\text{27.4}_{\pm \text{15.1}}$  \\
         Baichuan-turbo-192k$^\diamondsuit$ & $\text{14.0}_{\pm \text{5.8}}$ & $\text{34.4}_{\pm \text{11.0}}$ & $\text{46.2}_{\pm \text{14.6}}$ & $\text{61.8}_{\pm \text{17.1}}$ & $\text{9.3}_{\pm \text{4.7}}$ & $\text{21.7}_{\pm \text{13.7}}$ & $\text{30.9}_{\pm \text{17.9}}$ & $\text{41.4}_{\pm \text{21.9}}$  \\
         Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{14.0}_{\pm \text{5.8}}$ & $\text{25.0}_{\pm \text{11.8}}$ & $\text{32.4}_{\pm \text{10.0}}$ & $\text{49.5}_{\pm \text{8.5}}$ & $\text{2.0}_{\pm \text{3.2}}$ & $\text{5.0}_{\pm \text{7.1}}$ & $\text{5.2}_{\pm \text{6.5}}$ & $\text{8.8}_{\pm \text{6.0}}$  \\
    \bottomrule
    \end{tabular}
   }
    \label{exp:main_result}
\end{table}




% 10 authors non-topic ignore
\renewcommand{\arraystretch}{1.1}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{Evaluation result on Research Paper. Note: non-topic ignore}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c|cccc|cccc}
    \toprule
         & \multicolumn{8}{c}{\bf 10 authors} \\
         & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10} & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10}  \\
    \midrule
        GPT-4-turbo$^\diamondsuit$ & $\text{6.7}_{\pm \text{14.1}}$ & $\text{13.3}_{\pm \text{23.3}}$ & $\text{16.7}_{\pm \text{28.3}}$ & $\text{33.3}_{\pm \text{27.2}}$ & $\text{0.7}_{\pm \text{1.6}}$ & $\text{2.6}_{\pm \text{4.3}}$ & $\text{4.1}_{\pm \text{7.5}}$ & $\text{8.1}_{\pm \text{10.6}}$   \\
        Kimi$^\diamondsuit$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{16.7}_{\pm \text{17.6}}$ & $\text{16.7}_{\pm \text{17.6}}$ & $\text{30.0}_{\pm \text{18.9}}$ & $\text{1.1}_{\pm \text{1.8}}$ & $\text{2.2}_{\pm \text{2.6}}$ & $\text{2.2}_{\pm \text{2.6}}$ & $\text{4.8}_{\pm \text{3.5}}$   \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{46.7}_{\pm \text{35.8}}$ & $\text{56.7}_{\pm \text{31.6}}$ & $\text{56.7}_{\pm \text{31.6}}$ & $\text{63.3}_{\pm \text{24.6}}$ & $\text{5.2}_{\pm \text{3.9}}$ & $\text{13.7}_{\pm \text{7.0}}$ & $\text{21.1}_{\pm \text{10.3}}$ & $\text{34.4}_{\pm \text{16.8}}$   \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{3.3}_{\pm \text{10.5}}$ & $\text{6.7}_{\pm\text{14.1}}$ & $\text{16.7}_{\pm\text{17.6}}$ & $\text{33.3}_{\pm\text{27.2}}$ & $\text{0.4}_{\pm\text{1.2}}$ & $\text{1.5}_{\pm\text{3.6}}$ & $\text{3.3}_{\pm\text{5.6}}$ & $\text{7.4}_{\pm\text{10.9}}$   \\
    \midrule
        & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10}  & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10}  \\
    \midrule
        GPT-4-turbo$^\diamondsuit$ & $\text{6.7}_{\pm \text{14.1}}$ & $\text{7.8}_{\pm \text{12.9}}$ & $\text{7.3}_{\pm \text{13.5}}$ & $\text{7.3}_{\pm \text{9.5}}$ & $\text{13.3}_{\pm \text{2.8}}$ & $\text{38.9}_{\pm \text{64.4}}$ & $\text{5.2}_{\pm \text{9.6}}$ & $\text{7.7}_{\pm \text{10.0}}$  \\
        Kimi$^\diamondsuit$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{6.7}_{\pm \text{7.8}}$ & $\text{4.0}_{\pm \text{4.7}}$ & $\text{4.3}_{\pm \text{3.2}}$ & $\text{2.0}_{\pm \text{3.2}}$ & $\text{3.3}_{\pm \text{3.9}}$ & $\text{3.9}{\pm \text{3.3}}$ & $\text{4.6}{\pm \text{3.3}}$   \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{46.7}_{\pm\text{35.8}}$ & $\text{41.1}_{\pm\text{20.9}}$ & $\text{38.0}_{\pm\text{18.6}}$ & $\text{31.0}_{\pm\text{15.1}}$ & $\text{9.3}_{\pm\text{7.2}}$ & $\text{20.6}_{\pm\text{10.5}}$ & $\text{27.1}_{\pm\text{13.3}}$ & $\text{32.6}_{\pm\text{15.9}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{3.3}_{\pm\text{10.5}}$ & $\text{4.4}_{\pm\text{10.7}}$ & $\text{6.0}_{\pm\text{10.2}}$ & $\text{6.7}_{\pm\text{9.8}}$ & $\text{0.7}_{\pm\text{2.1}}$ & $\text{2.2}_{\pm\text{5.4}}$ & $\text{4.3}_{\pm\text{7.3}}$ & $\text{7.0}_{\pm\text{10.3}}$   \\

    \bottomrule
    \end{tabular}
   }
    \label{exp:main_result}
\end{table}

==> table/ap_paper-eval-topic-ignored.tex <==
%%% evaluation
\renewcommand{\arraystretch}{1.2}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{Evaluation result on Research Paper.Note: topic ignore}
    \resizebox{1.1\textwidth}{!}
    {
    \begin{tabular}{c|cccc|cccc}
    \toprule
         & \multicolumn{4}{c}{\bf 2 authors} & \multicolumn{4}{c}{\bf 5 authors}  \\
         & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10} & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10}  \\
    \midrule
         GPT-3.5-turbo$^\diamondsuit$ & $\text{70.0}_{\pm \text{24.6}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{46.7}_{\pm \text{23.3}}$ & $\text{70.0}_{\pm \text{24.6}}$ & $\text{83.3}_{\pm \text{17.6}}$  \\
         GPT-4-turbo$^\diamondsuit$ & $\text{83.3}_{\pm \text{32.4}}$ & $\text{93.3}_{\pm \text{14.1}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{53.3}_{\pm \text{23.3}}$ & $\text{80.0}_{\pm \text{17.2}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{96.7}_{\pm \text{10.5}}$ \\ 
         Kimi$^\diamondsuit$ & $\text{83.3}_{\pm \text{17.5}}$ & $\text{83.3}_{\pm \text{17.5}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{96.7}_{\pm \text{10.5}}$ & $\text{43.3}_{\pm \text{27.4}}$ & $\text{53.3}_{\pm \text{28.1}}$ & $\text{60.0}_{\pm \text{21.1}}$ & $\text{76.7}_{\pm \text{16.1}}$  \\
         Baichuan-turbo-192k$^\diamondsuit$ & $\text{60.0}_{\pm \text{30.6}}$ & $\text{70.0}_{\pm \text{24.6}}$ & $\text{70.0}_{\pm \text{24.6}}$ & $\text{76.7}_{\pm \text{26.3}}$ & $\text{36.7}_{\pm \text{24.6}}$ & $\text{46.7}_{\pm \text{23.3}}$ & $\text{63.3}_{\pm \text{22.5}}$ & $\text{73.3}_{\pm \text{22.5}}$  \\
         Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{56.7}_{\pm \text{22.5}}$ & $\text{76.7}_{\pm \text{22.5}}$ & $\text{86.7}_{\pm \text{17.2}}$ & $\text{90.0}_{\pm \text{16.1}}$ & $\text{13.3}_{\pm \text{17.2}}$ & $\text{23.3}_{\pm \text{22.5}}$ & $\text{33.3}_{\pm \text{27.2}}$ & $\text{73.3}_{\pm \text{30.6}}$  \\
    \midrule
        & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} \\
    \midrule
        GPT-3.5-turbo$^\diamondsuit$ & $\text{70.0}_{\pm \text{24.6}}$ & $\text{68.9}_{\pm \text{21.5}}$ & $\text{60.0}_{\pm \text{14.7}}$ & $\text{49.0}_{\pm \text{7.4}}$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{17.8}_{\pm \text{10.7}}$ & $\text{20.0}_{\pm \text{9.4}}$ & $\text{18.0}_{\pm \text{6.5}}$  \\
        GPT-4-turbo$^\diamondsuit$ & $\text{83.3}_{\pm \text{32.4}}$ & $\text{73.3}_{\pm \text{21.7}}$ & $\text{70.7}_{\pm \text{10.5}}$ & $\text{54.7}_{\pm \text{7.2}}$ & $\text{53.3}_{\pm \text{23.3}}$ & $\text{43.3}_{\pm \text{9.7}}$ & $\text{33.3}_{\pm \text{7.0}}$ & $\text{27.7}_{\pm \text{5.7}}$  \\
        Kimi$^\diamondsuit$ & $\text{83.3}_{\pm \text{17.5}}$ & $\text{70.2}_{\pm \text{21.6}}$ & $\text{64.7}_{\pm \text{23.1}}$ & $\text{56.1}_{\pm \text{15.1}}$ & $\text{43.3}_{\pm \text{27.4}}$ & $\text{30.1}_{\pm \text{15.8}}$ & $\text{20.0}_{\pm \text{10.4}}$ & $\text{17.4}_{\pm \text{5.3}}$  \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{60.0}_{\pm \text{30.6}}$ & $\text{60.0}_{\pm \text{26.8}}$ & $\text{58.0}_{\pm \text{24.2}}$ & $\text{48.0}_{\pm \text{19.7}}$ & $\text{36.7}_{\pm \text{24.6}}$ & $\text{33.3}_{\pm \text{20.9}}$ & $\text{30.0}_{\pm \text{18.1}}$ & $\text{30.7}_{\pm \text{18.7}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{56.7}_{\pm \text{22.5}}$ & $\text{51.1}_{\pm \text{19.7}}$ & $\text{46.7}_{\pm \text{12.2}}$ & $\text{41.0}_{\pm \text{8.6}}$ & $\text{13.3}_{\pm \text{17.2}}$ & $\text{8.9}_{\pm \text{8.8}}$ & $\text{8.0}_{\pm \text{6.9}}$ & $\text{12.0}_{\pm \text{5.9}}$  \\
    \midrule
        & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} \\
    \midrule
        GPT-3.5-turbo$^\diamondsuit$ & $\text{7.8}_{\pm \text{2.7}}$ & $\text{23.0}_{\pm \text{7.2}}$ & $\text{33.3}_{\pm \text{8.2}}$ & $\text{54.4}_{\pm \text{8.2}}$ & $\text{1.1}_{\pm \text{1.8}}$ & $\text{5.9}_{\pm \text{3.6}}$ & $\text{11.1}_{\pm \text{5.2}}$ & $\text{20.0}_{\pm \text{7.2}}$  \\
        GPT-4-turbo$^\diamondsuit$ & $\text{9.3}_{\pm \text{3.6}}$ & $\text{24.4}_{\pm \text{7.2}}$ & $\text{39.3}_{\pm \text{5.8}}$ & $\text{60.7}_{\pm \text{8.0}}$ & $\text{5.9}_{\pm \text{2.6}}$ & $\text{14.4}_{\pm \text{3.2}}$ & $\text{18.5}_{\pm \text{3.9}}$ & $\text{30.7}_{\pm \text{6.3}}$  \\
        Kimi$^\diamondsuit$ & $\text{9.3}_{\pm \text{2.0}}$ & $\text{23.3}_{\pm \text{7.2}}$ & $\text{35.9}_{\pm \text{12.8}}$ & $\text{62.2}_{\pm \text{16.7}}$ & $\text{4.8}_{\pm \text{3.1}}$ & $\text{10.0}_{\pm \text{5.3}}$ & $\text{12.2}_{\pm \text{5.8}}$ & $\text{18.9}_{\pm \text{5.9}}$   \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{6.7}_{\pm \text{3.4}}$ & $\text{20.0}_{\pm \text{8.9}}$ & $\text{32.2}_{\pm \text{13.4}}$ & $\text{53.3}_{\pm \text{21.9}}$ & $\text{4.1}_{\pm \text{2.7}}$ & $\text{11.1}_{\pm \text{7.0}}$ & $\text{19.3}_{\pm \text{10.1}}$ & $\text{34.1}_{\pm \text{20.8}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{6.3}_{\pm \text{2.5}}$ & $\text{17.0}_{\pm \text{6.6}}$ & $\text{25.9}_{\pm \text{6.8}}$ & $\text{45.6}_{\pm \text{9.6}}$ & $\text{1.5}_{\pm \text{1.9}}$ & $\text{3.0}_{\pm \text{2.9}}$ & $\text{4.4}_{\pm \text{3.8}}$ & $\text{13.3}_{\pm \text{6.6}}$  \\
    \midrule
        & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} \\
    \midrule
        GPT-3.5-turbo$^\diamondsuit$ & $\text{14.0}_{\pm \text{4.9}}$ & $\text{34.4}_{\pm \text{10.7}}$ & $\text{42.9}_{\pm \text{10.5}}$ & $\text{51.6}_{\pm \text{7.8}}$ & $\text{2.0}_{\pm \text{3.2}}$ & $\text{8.9}_{\pm \text{5.4}}$ & $\text{14.3}_{\pm \text{6.7}}$ & $\text{18.9}_{\pm \text{6.9}}$  \\
        GPT-4-turbo$^\diamondsuit$ & $\text{16.7}_{\pm \text{6.5}}$ & $\text{36.7}_{\pm \text{10.9}}$ & $\text{50.5}_{\pm \text{7.5}}$ & $\text{57.5}_{\pm \text{7.6}}$& $\text{10.7}_{\pm \text{4.7}}$ & $\text{21.7}_{\pm \text{4.9}}$ & $\text{23.8}_{\pm \text{5.0}}$ & $\text{29.1}_{\pm \text{6.0}}$  \\
        Kimi$^\diamondsuit$ & $\text{16.7}_{\pm \text{3.5}}$ & $\text{35.0}_{\pm \text{10.8}}$ & $\text{46.2}_{\pm \text{16.5}}$ & $\text{58.9}_{\pm \text{15.9}}$ & $\text{8.7}_{\pm \text{5.5}}$ & $\text{15.0}_{\pm \text{7.9}}$ & $\text{15.7}_{\pm \text{7.5}}$ & $\text{17.9}_{\pm \text{5.6}}$  \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{12.0}_{\pm \text{6.1}}$ & $\text{30.0}_{\pm \text{13.4}}$ & $\text{41.4}_{\pm \text{17.3}}$ & $\text{50.5}_{\pm \text{20.7}}$ & $\text{7.3}_{\pm \text{4.9}}$ & $\text{16.7}_{\pm \text{10.5}}$ & $\text{24.8}_{\pm \text{12.9}}$ & $\text{32.3}_{\pm \text{19.7}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{6.3}_{\pm \text{2.5}}$ & $\text{17.0}_{\pm \text{6.6}}$ & $\text{25.9}_{\pm \text{6.8}}$ & $\text{45.6}_{\pm \text{9.6}}$ & $\text{2.7}_{\pm \text{3.4}}$ & $\text{4.4}_{\pm \text{4.4}}$ & $\text{5.7}_{\pm \text{4.9}}$ & $\text{12.6}_{\pm \text{6.2}}$  \\
    \bottomrule
    \end{tabular}
   }
    \label{exp:main_result}
\end{table}





% 10 authors
\renewcommand{\arraystretch}{1.2}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{Evaluation result on Research Paper. Note: topic ignore}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c|cccc|cccc}
    \toprule
         & \multicolumn{8}{c}{\bf 10 authors} \\
         & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10} & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10}  \\
    \midrule
        GPT-4-turbo$^\diamondsuit$ & $\text{23.3}_{\pm \text{27.4}}$ & $\text{30.0}_{\pm \text{29.2}}$ & $\text{36.7}_{\pm \text{24.6}}$ & $\text{50.2}_{\pm \text{23.5}}$ & $\text{2.6}_{\pm \text{3.0}}$ & $\text{4.8}_{\pm \text{5.3}}$ & $\text{5.9}_{\pm \text{5.6}}$ & $\text{10.4}_{\pm \text{8.7}}$   \\
        Kimi$^\diamondsuit$ & $\text{20.0}_{\pm \text{23.3}}$ & $\text{40.0}_{\pm \text{30.6}}$ & $\text{40.0}_{\pm \text{30.6}}$ & $\text{56.7}_{\pm \text{22.5}}$ & $\text{2.2}_{\pm \text{2.6}}$ & $\text{4.8}_{\pm \text{5.5}}$ & $\text{5.9}_{\pm \text{7.4}}$ & $\text{5.9}_{\pm \text{7.4}}$   \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{36.7}_{\pm \text{24.6}}$ & $\text{46.7}_{\pm \text{32.2}}$ & $\text{56.7}_{\pm \text{33.2}}$ & $\text{66.7}_{\pm \text{31.4}}$ & $\text{4.1}_{\pm \text{2.7}}$ & $\text{10.0}_{\pm \text{9.1}}$ & $\text{16.7}_{\pm \text{15.4}}$ & $\text{30.7}_{\pm \text{25.4}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{23.3}_{\pm \text{22.5}}$ & $\text{23.3}_{\pm \text{22.5}}$ & $\text{36.7}_{\pm \text{18.9}}$ & $\text{1.1}_{\pm \text{1.8}}$ & $\text{3.3}_{\pm \text{3.7}}$ & $\text{4.8}_{\pm \text{6.1}}$ & $\text{10.4}_{\pm \text{11.7}}$  \\
    \midrule
        & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10}  & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10}  \\
    \midrule
        GPT-4-turbo$^\diamondsuit$ & $\text{23.3}_{\pm \text{27.4}}$ & $\text{14.4}_{\pm \text{15.8}}$ & $\text{10.7}_{\pm \text{10.0}}$ & $\text{9.3}_{\pm \text{7.9}}$ & $\text{4.7}_{\pm \text{5.5}}$ & $\text{7.2}_{\pm \text{7.9}}$ & $\text{7.6}_{\pm \text{7.2}}$ & $\text{9.8}_{\pm \text{8.4}}$  \\
        Kimi$^\diamondsuit$ & $\text{20.0}_{\pm \text{23.3}}$ & $\text{14.4}_{\pm \text{16.6}}$ & $\text{10.7}_{\pm \text{13.4}}$ & $\text{9.3}_{\pm \text{7.0}}$ & $\text{4.0}_{\pm \text{4.7}}$ & $\text{7.2}_{\pm \text{8.3}}$ & $\text{7.6}_{\pm \text{9.6}}$ & $\text{9.8}_{\pm \text{7.4}}$  \\
        Baichuan-turbo-192k$^\diamondsuit$ & $\text{36.7}_{\pm \text{24.6}}$ & $\text{30.0}_{\pm \text{27.2}}$ & $\text{30.0}_{\pm \text{27.7}}$ & $\text{27.7}_{\pm \text{22.8}}$ & $\text{7.3}_{\pm \text{4.9}}$ & $\text{15.0}_{\pm \text{13.6}}$ & $\text{21.4}_{\pm \text{19.8}}$ & $\text{29.1}_{\pm \text{24.0}}$  \\
        Qwen1.5-72B-Chat$^\diamondsuit$ & $\text{10.0}_{\pm \text{16.1}}$ & $\text{10.0}_{\pm \text{11.0}}$ & $\text{8.7}_{\pm \text{10.9}}$ & $\text{9.3}_{\pm \text{10.5}}$ & $\text{2.0}_{\pm \text{3.2}}$ & $\text{5.0}_{\pm \text{5.5}}$ & $\text{6.2}_{\pm \text{7.8}}$ & $\text{9.8}_{\pm \text{11.1}}$  \\

    \bottomrule
    \end{tabular}
   }
    \label{exp:main_result}
\end{table}

==> table/ap_searching_2_5authors.tex <==
\renewcommand{\arraystretch}{1.1}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{searching...}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c|ccc|ccc}
    \toprule
         % & \multicolumn{3}{c}{\bf 2 authors} & \multicolumn{3}{c}{\bf 5 authors}  \\
          & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5}   \\
    \midrule
         \textbf{2 authors} & $\text{70.0}_{\pm \text{33.1}}$ & $\text{93.3}_{\pm \text{14.1}}$ & $\text{96.7}_{\pm \text{10.5}}$ & $\text{70.0}_{\pm \text{33.1}}$ & $\text{61.1}_{\pm \text{20.5}}$ & $\text{55.3}_{\pm \text{16.6}}$  \\
    \midrule
         \textbf{5 authors} & $\text{46.0}_{\pm \text{26.7}}$ & $\text{80.0}_{\pm \text{13.3}}$ & $\text{90.0}_{\pm \text{14.1}}$ & $\text{46.0}_{\pm \text{26.7}}$ & $\text{41.3}_{\pm \text{14.3}}$ & $\text{36.8}_{\pm \text{9.9}}$  \\
    \bottomrule
    \end{tabular}
   }
    \label{exp:searching}
\end{table}




==> table/ap_searching_vs_pipeline.tex <==
%%%% baseline vs. RAG-based pipeline
\renewcommand{\arraystretch}{1.2}
% \addtolength{\tabcolsep}{-1.5pt} 
\begin{table}[h!]
    \centering
    \caption{baseline vs. RAG-based pipeline}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c|cccc|cccc}
    \toprule
         & \multicolumn{4}{c}{\bf 50 papers filter 10 papers} & \multicolumn{4}{c}{\bf 200 papers filter 50 papers}  \\
         & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10} & \textbf{Rank@1} & \textbf{Rank@3} & \textbf{Rank@5} & \textbf{Rank@10}  \\
    \midrule
         Searching & $\text{46.0}_{\pm \text{26.7}}$ & $\text{80.0}_{\pm \text{13.3}}$ & $\text{90.0}_{\pm \text{14.1}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{10.0}_{\pm \text{14.1}}$ & $\text{18.0}_{\pm \text{11.4}}$ & $\text{26.0}_{\pm \text{13.5}}$ & $\text{84.0}_{\pm \text{12.6}}$  \\
         \rowcolor{gray!30} RAG+Qwen & $\text{54.0}_{\pm \text{25.0}}$ & $\text{78.0}_{\pm \text{11.4}}$ & $\text{94.0}_{\pm \text{9.7}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{14.0}_{\pm \text{13.5}}$ & $\text{22.3}_{\pm \text{14.7}}$ & $\text{26.1}_{\pm \text{18.3}}$ &  $\text{36.0}_{\pm \text{18.4}}$ \\ 
         \rowcolor{gray!30} RAG+GPT-3.5-turbo & $\text{40.0}_{\pm \text{16.3}}$ & $\text{72.0}_{\pm \text{16.9}}$ & $\text{86.0}_{\pm \text{13.5}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{2.0}_{\pm \text{6.3}}$ & $\text{12.0}_{\pm \text{16.8}}$ & $\text{16.0}_{\pm \text{20.1}}$ & $\text{30.0}_{\pm \text{23.6}}$  \\
         \rowcolor{gray!30} RAG+GPT-4-turbo & $\text{54.0}_{\pm \text{23.0}}$ & $\text{76.0}_{\pm \text{18.0}}$ & $\text{84.0}_{\pm \text{13.0}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{40.0}_{\pm \text{31.3}}$ & $\text{52.0}_{\pm \text{25.3}}$ & $\text{56.0}_{\pm \text{22.7}}$ & $\text{72.0}_{\pm \text{23.5}}$  \\
         \rowcolor{gray!30} RAG+Kimi & $\text{64.0}_{\pm \text{20.7}}$ & $\text{76.0}_{\pm \text{15.8}}$ & $\text{86.0}_{\pm \text{13.5}}$ & $\text{100.0}_{\pm \text{0.0}}$ & $\text{50.0}_{\pm \text{28.7}}$ & $\text{60.0}_{\pm \text{28.3}}$ & $\text{64.0}_{\pm \text{26.3}}$ & $\text{82.0}_{\pm \text{14.8}}$  \\
         RAG+Baichuan & $\text{48.0}_{\pm \text{14.0}}$ & $\text{74.0}_{\pm \text{21.2}}$ & $\text{82.0}_{\pm \text{19.9}}$ & $\text{82.0}_{\pm \text{19.9}}$ & $\text{8.0}_{\pm \text{19.3}}$ & $\text{12.0}_{\pm \text{21.5}}$ & $\text{14.0}_{\pm \text{21.2}}$ & $\text{22.0}_{\pm \text{25.7}}$  \\
    \midrule
        & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} & \textbf{Precision@1} & \textbf{Precision@3} & \textbf{Precision@5} & \textbf{Precision@10} \\
    \midrule
         Searching & $\text{46.0}_{\pm \text{26.7}}$ & $\text{41.3}_{\pm \text{14.3}}$ & $\text{36.8}_{\pm \text{9.9}}$ & $\text{30.8}_{\pm \text{3.3}}$ & $\text{10.0}_{\pm \text{14.1}}$ & $\text{8.7}_{\pm \text{5.5}}$ & $\text{7.6}_{\pm \text{4.4}}$ & $\text{5.8}_{\pm \text{3.3}}$  \\
         \rowcolor{gray!30} RAG+Qwen & $\text{54.0}_{\pm \text{25.0}}$ & $\text{41.3}_{\pm \text{8.2}}$ & $\text{35.2}_{\pm \text{4.1}}$ & $\text{30.8}_{\pm \text{3.3}}$ & $\text{14.0}_{\pm \text{13.5}}$ & $\text{11.3}_{\pm \text{8.3}}$ & $\text{7.6}_{\pm \text{5.8}}$ & $\text{5.2}_{\pm \text{3.0}}$  \\ 
         \rowcolor{gray!30} RAG+GPT-3.5-turbo & $\text{40.0}_{\pm \text{16.3}}$ & $\text{40.7}_{\pm \text{8.6}}$ & $\text{36.4}_{\pm \text{6.1}}$ & $\text{30.8}_{\pm \text{3.3}}$ & $\text{2.0}_{\pm \text{6.3}}$ & $\text{4.0}_{\pm \text{5.6}}$ & $\text{4.0}_{\pm \text{4.6}}$ & $\text{3.8}_{\pm \text{3.0}}$  \\
         \rowcolor{gray!30} RAG+GPT-4-turbo & $\text{54.0}_{\pm \text{23.0}}$ & $\text{44.7}_{\pm \text{15.7}}$ & $\text{37.6}_{\pm \text{9.7}}$ & $\text{30.8}_{\pm \text{3.3}}$ & $\text{40.0}_{\pm \text{31.3}}$ & $\text{25.3}_{\pm \text{16.6}}$ & $\text{20.0}_{\pm \text{11.0}}$ & $\text{14.2}_{\pm \text{5.6}}$  \\
         \rowcolor{gray!30} RAG+Kimi & $\text{64.0}_{\pm \text{20.7}}$ & $\text{50.0}_{\pm \text{9.6}}$ & $\text{39.2}_{\pm \text{9.2}}$ & $\text{30.8}_{\pm \text{3.3}}$ & $\text{50.0}_{\pm \text{28.7}}$ & $\text{38.7}_{\pm \text{24.3}}$ & $\text{28.4}_{\pm \text{17.2}}$ & $\text{19.2}_{\pm \text{7.4}}$  \\
         RAG+Baichuan & $\text{48.0}_{\pm \text{14.0}}$ & $\text{47.3}_{\pm \text{15.5}}$ & $\text{36.4}_{\pm \text{10.7}}$ & $\text{18.2}_{\pm \text{5.4}}$ & $\text{8.0}_{\pm \text{19.3}}$ & $\text{8.0}_{\pm \text{16.9}}$ & $\text{5.2}_{\pm \text{10.0}}$ & $\text{4.2}_{\pm \text{5.8}}$  \\
    \midrule
        & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} & \textbf{Recall@1} & \textbf{Recall@3} & \textbf{Recall@5} & \textbf{Recall@10} \\
    \midrule
         Searching & $\text{5.1}_{\pm \text{2.9}}$ & $\text{13.8}_{\pm \text{4.7}}$ & $\text{20.4}_{\pm \text{5.5}}$ & $\text{34.2}_{\pm \text{3.7}}$ & $\text{1.1}_{\pm \text{1.6}}$ & $\text{2.9}_{\pm \text{1.8}}$ & $\text{4.2}_{\pm \text{2.4}}$ & $\text{6.4}_{\pm \text{3.7}}$  \\
         \rowcolor{gray!30} RAG+Qwen & $\text{6.0}_{\pm \text{2.7}}$ & $\text{13.8}_{\pm \text{2.7}}$ & $\text{19.6}_{\pm \text{2.3}}$ & $\text{34.2}_{\pm \text{3.7}}$ & $\text{1.6}_{\pm \text{1.5}}$ & $\text{3.8}_{\pm \text{2.7}}$ & $\text{4.2}_{\pm \text{3.2}}$ & $\text{5.8}_{\pm \text{3.3}}$  \\ 
         \rowcolor{gray!30} RAG+GPT-3.5-turbo & $\text{4.4}_{\pm \text{1.8}}$ & $\text{13.6}_{\pm \text{2.9}}$ & $\text{20.2}_{\pm \text{3.4}}$ & $\text{34.2}_{\pm \text{3.7}}$ & $\text{0.2}_{\pm \text{0.7}}$ & $\text{1.3}_{\pm \text{1.9}}$ & $\text{2.2}_{\pm \text{3.1}}$ & $\text{4.2}_{\pm \text{3.4}}$  \\
         \rowcolor{gray!30} RAG+GPT-4-turbo & $\text{6.0}_{\pm \text{3.0}}$ & $\text{14.9}_{\pm \text{5.2}}$ & $\text{20.9}_{\pm \text{5.4}}$ & $\text{34.2}_{\pm \text{3.7}}$ & $\text{4.4}_{\pm \text{3.5}}$ & $\text{8.4}_{\pm \text{5.5}}$ & $\text{11.1}_{\pm \text{6.1}}$ & $\text{15.8}_{\pm \text{6.2}}$  \\
         \rowcolor{gray!30} RAG+Kimi & $\text{7.1}_{\pm \text{2.3}}$ & $\text{16.7}_{\pm \text{3.2}}$ & $\text{21.8}_{\pm \text{5.1}}$ & $\text{34.2}_{\pm \text{3.7}}$ & $\text{5.6}_{\pm \text{3.2}}$ & $\text{12.9}_{\pm \text{8.1}}$ & $\text{15.8}_{\pm \text{9.6}}$ & $\text{21.3}_{\pm \text{8.3}}$  \\
         RAG+Baichuan & $\text{5.3}_{\pm \text{1.6}}$ & $\text{15.8}_{\pm \text{5.2}}$ & $\text{20.2}_{\pm \text{6.0}}$ & $\text{20.2}_{\pm \text{6.0}}$ & $\text{0.9}_{\pm \text{2.1}}$ & $\text{2.7}_{\pm \text{5.6}}$ & $\text{2.9}_{\pm \text{5.5}}$ & $\text{4.7}_{\pm \text{6.4}}$   \\
    \midrule
        & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} & \textbf{F1-score@1} & \textbf{F1-score@3} & \textbf{F1-score@5} & \textbf{F1-score@10} \\
    \midrule
         Searching & $\text{9.1}_{\pm \text{5.3}}$ & $\text{20.6}_{\pm \text{7.2}}$ & $\text{26.3}_{\pm \text{7.1}}$ & $\text{32.4}_{\pm \text{3.5}}$ & $\text{2.0}_{\pm \text{2.8}}$ & $\text{4.3}_{\pm \text{2.7}}$ & $\text{5.4}_{\pm \text{3.1}}$ & $\text{6.1}_{\pm \text{3.5}}$  \\
         \rowcolor{gray!30} RAG+Qwen & $\text{10.8}_{\pm \text{5.0}}$ & $\text{20.1}_{\pm \text{4.1}}$ & $\text{25.1}_{\pm \text{2.9}}$ & $\text{32.4}_{\pm \text{3.5}}$ & $\text{2.8}_{\pm \text{2.7}}$ & $\text{5.7}_{\pm \text{4.1}}$ & $\text{5.4}_{\pm \text{4.1}}$ & $\text{5.5}_{\pm \text{3.2}}$  \\ 
         \rowcolor{gray!30} RAG+GPT-3.5-turbo & $\text{8.0}_{\pm \text{3.3}}$ & $\text{20.3}_{\pm \text{4.3}}$ & $\text{26.0}_{\pm \text{4.4}}$ & $\text{32.4}_{\pm \text{3.5}}$ & $\text{0.4}_{\pm \text{1.3}}$ & $\text{2.0}_{\pm \text{2.8}}$ & $\text{2.9}_{\pm \text{4.0}}$ & $\text{4.0}_{\pm \text{3.2}}$  \\
         \rowcolor{gray!30} RAG+GPT-4-turbo & $\text{10.8}_{\pm \text{4.6}}$ & $\text{22.3}_{\pm \text{7.9}}$ & $\text{26.9}_{\pm \text{6.9}}$ & $\text{32.4}_{\pm \text{3.5}}$ & $\text{8.0}_{\pm \text{6.3}}$ & $\text{12.7}_{\pm \text{8.3}}$ & $\text{14.3}_{\pm \text{7.9}}$ & $\text{14.9}_{\pm \text{5.9}}$  \\
         \rowcolor{gray!30} RAG+Kimi & $\text{12.8}_{\pm \text{4.1}}$ & $\text{25.0}_{\pm \text{4.8}}$ & $\text{28.0}_{\pm \text{6.6}}$ & $\text{32.4}_{\pm \text{3.5}}$ & $\text{10.0}_{\pm \text{5.7}}$ & $\text{19.3}_{\pm \text{12.2}}$ & $\text{20.3}_{\pm \text{12.3}}$ & $\text{20.2}_{\pm \text{7.8}}$  \\
         RAG+Baichuan & $\text{9.6}_{\pm \text{2.8}}$ & $\text{23.7}_{\pm \text{7.8}}$ & $\text{26.0}_{\pm \text{7.7}}$ & $\text{19.2}_{\pm \text{5.7}}$ & $\text{1.6}_{\pm \text{3.9}}$ & $\text{4.0}_{\pm \text{8.4}}$ & $\text{3.7}_{\pm \text{7.1}}$ & $\text{4.4}_{\pm \text{6.1}}$   \\
    \bottomrule
    \end{tabular}
   }
    \label{exp:main_result}
\end{table}
